A possible 250-second X-ray quasi-periodicity in the fast blue optical transient AT2018cow

The fast blue optical transients (FBOTs) are a new population of extragalactic transients of unclear physical origin. A variety of mechanisms have been proposed including failed supernova explosion, shock interaction with a dense medium, young magnetar, accretion onto a compact object, and stellar tidal disruption event, but none is conclusive. Here we report the discovery of a possible X-ray quasi-periodicity signal with a period of $\sim$250 second (at a significance level of 99.76%) in the brightest FBOT AT2018cow through the analysis of XMM-Newton/PN data. The signal is independently detected at the same frequency in the average power density spectrum from data taken from the Swift telescope, with observations covering from 6 to 37 days after the optical discovery, though the significance level is lower (94.26%). This suggests that the QPO frequency may be stable over at least 1.1$\times$ 10$^{4}$ cycles. Assuming the $\sim$250 second QPO to be a scaled-down analogue of that typically seen in stellar mass black holes, a black hole mass of $\sim10^{3}-10^{5}$ solar masses could be inferred. The overall X-ray luminosity evolution could be modeled with the stellar tidal disruption by a black hole of $\sim10^4$ solar masses, providing a viable mechanism to produce AT2018cow. Our findings suggest that other bright FBOTs may also harbor intermediate-mass black holes.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

